LocalTweets to LocalHealth: A Mental Health Surveillance Framework Based on Twitter Data

Prior research on Twitter (now X) data has provided positive evidence of its utility in developing supplementary health surveillance systems. In this study, we present a new framework to surveil public health, focusing on mental health (MH) outcomes. We hypothesize that locally posted tweets are indicative of local MH outcomes and collect tweets posted from 765 neighborhoods (census block groups) in the USA. We pair these tweets from each neighborhood with the corresponding MH outcome reported by the Center for Disease Control (CDC) to create a benchmark dataset, LocalTweets. With LocalTweets, we present the first population-level evaluation task for Twitter-based MH surveillance systems. We then develop an efficient and effective method, LocalHealth, for predicting MH outcomes based on LocalTweets. When used with GPT3.5, LocalHealth achieves the highest F1-score and accuracy of 0.7429 and 79.78\%, respectively, a 59\% improvement in F1-score over the GPT3.5 in zero-shot setting. We also utilize LocalHealth to extrapolate CDC's estimates to proxy unreported neighborhoods, achieving an F1-score of 0.7291. Our work suggests that Twitter data can be effectively leveraged to simulate neighborhood-level MH outcomes.

==> tables/table_result_1_with_stat_sig.tex <==
% table_result_1.tex

\begin{table}
\caption{Performance Metrics}
\centering
\begin{tabularx}{\linewidth}{ccccc}
\toprule
\textbf{Year} & \textbf{MH} & \textbf{FI} & \textbf{General} & \textbf{ADI} \\
\midrule

2015 & 0.1640*** & 0.1460*** & 0.1299*** & 0.6767*** \\
2016 & 0.1366*** & 0.1332*** & 0.1215*** & 0.7074*** \\
2017 & 0.1123** & 0.1132** & 0.0969** & 0.7257*** \\
2018 & 0.0928* & 0.0937** & 0.0863* & 0.7162*** \\
2019 & 0.0922* & 0.0954** & 0.0832* & 0.7318*** \\

\bottomrule
\end{tabularx}
\end{table}

==> tables/table_result_2_extended.tex <==
% table_result_2.tex

\begin{table*}
\caption{Performance Metrics}
\centering
\begin{tabularx}{\linewidth}{Xcccccc}
\toprule
\textbf{Input information} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Accuracy} \\
\midrule
\textbf{Baseline 1: Majority baseline (All low-risk)} & 0.3828 & 0.5000 & 0.4336 & 0.7656 \\
\midrule
\textbf{Baseline 2: ADI-only (Linear Regression)} & 0.6421 (0.14) & 0.7194 (0.12) & 0.6406 (0.11) & 0.7281 (0.05) \\
\midrule
\textbf{Baseline 3: Text-based model (Logistic Regression)} & & & & \\
MH only & 0.5908 (0.01) & 0.5715 (0.01) & 0.3801 (0.02) & 0.3830 (0.02) \\
FI only & 0.5787 (0.00) & 0.5846 (0.00) & 0.4410 (0.01) & 0.4414 (0.01) \\
MH and FI & 0.5927 (0.04) & 0.5900 (0.05) & 0.4693 (0.01) & 0.5216 (0.11) \\
General only & 0.6212 (0.00) & 0.6493 (0.01) & 0.5224 (0.01) & 0.5275 (0.01) \\

\midrule
\textbf{Baseline 4: Text-based model (Support Vector Machine)} & & & & \\
MH only & 0.5830 (0.00) & 0.5171 (0.00) & 0.4839 (0.00) & 0.7516 (0.00) \\
FI only & 0.5327 (0.00) & 0.5074 (0.00) & 0.4711 (0.00) & 0.7425 (0.00) \\
MH and FI & 0.6161 (0.00) & 0.5224 (0.00) & 0.4908 (0.00) & 0.7569 (0.00) \\
General only & 0.6709 (0.00) & 0.5572 (0.00) & 0.5510 (0.00) & 0.7673 (0.00) \\

\midrule
\textbf{Count-based model} & & & & \\
MH only & 0.5170 (0.06) & 0.5356 (0.03) & 0.5052 (0.04) & 0.6195 (0.08) \\
FI only & 0.4411 (0.02) & 0.4751 (0.01) & 0.4465 (0.01) & 0.6788 (0.06) \\
MH and FI & 0.5239 (0.03) & 0.5261 (0.03) & 0.5133 (0.03) & 0.6384 (0.06) \\
General only & -- & -- & -- & -- \\

\midrule
\textbf{Text-based model} & & & & \\
MH only & 0.5917 (0.01) & 0.6247 (0.02) & 0.5668 (0.02) & 0.6005 (0.02) \\
FI only & 0.5620 (0.01) & 0.5738 (0.02) & 0.5602 (0.01) & 0.6443 (0.02) \\
MH and FI & 0.5905 (0.02) & 0.6170 (0.02) & 0.5853 (0.02) & 0.6416 (0.03) \\
General only & 0.5965 (0.01) & 0.6194 (0.02) & 0.5984 (0.01) & 0.6676 (0.01) \\

\midrule
\textbf{Text and Count-based model} & & & & \\
MH only & 0.5709 (0.04) & 0.5951 (0.05) & 0.5515 (0.03) & 0.6075 (0.04) \\
FI only & 0.5489 (0.05) & 0.5596 (0.05) & 0.5481 (0.05) & 0.6599 (0.04) \\
MH and FI & 0.5803 (0.02) & 0.6067 (0.03) & 0.5681 (0.02) & 0.6187 (0.02) \\
General only & 0.5752 (0.04) & 0.5942 (0.05) & 0.5732 (0.05) & 0.6639 (0.03) \\
\midrule

\midrule
\textbf{Count-based with ADI} & & & & \\
MH-only & 0.5628 (0.15) & 0.6328 (0.14) & 0.5647 (0.12) & 0.6936 (0.04) \\
FI only & 0.5519 (0.15) & 0.6173 (0.14) & 0.5545 (0.13) & 0.7157 (0.04) \\
MH and FI & 0.6267 (0.12) & 0.6966 (0.11) & 0.6138 (0.10) & 0.6931 (0.03) \\
General only & -- & -- & -- & -- \\

\midrule
\textbf{Text-based with ADI} & & & & \\
MH only & 0.7127 (0.02) & 0.7697 (0.01) & 0.7089 (0.04) & 0.7452 (0.05) \\
FI only & 0.7092 (0.02) & 0.7633 (0.03) & 0.7117 (0.03) & 0.7536 (0.04) \\
MH and FI & 0.7093 (0.02) & 0.7719 (0.01) & 0.7085 (0.03) & 0.7433 (0.04) \\
General only & 0.7189 (0.01) & 0.7735 (0.01) & 0.7236 (0.02) & 0.7648 (0.03) \\

\midrule
\textbf{Text-based with ADI and Sentiment} & & & & \\
MH only & 0.7053 (0.02) & 0.7667 (0.01) & 0.7013 (0.03) & 0.7358 (0.04) \\
FI only & 0.7099 (0.01) & 0.7679 (0.01) & 0.7133 (0.02) & 0.7529 (0.03) \\
MH and FI & 0.6984 (0.02) & 0.7631 (0.02) & 0.6895 (0.03) & 0.7205 (0.04) \\
General only & 0.7194 (0.01) & 0.7798 (0.01) & 0.7254 (0.02) & 0.7639 (0.03) \\

\bottomrule
\end{tabularx}
\end{table*}


==> tables/table_result_2_small_extended.tex <==
% table_result_2.tex

\begin{table}
\caption{Performance Metrics}
\centering
\begin{tabularx}{\linewidth}{Xccc}
\toprule
\textbf{Input information} & \textbf{F1-score} & \textbf{Accuracy} \\
\midrule
\textbf{Majority baseline}  & 0.4336 & 0.7656 \\
\textbf{ADI-only (Lin. Reg.)} & 0.6406 (0.11) & 0.7281 (0.05) \\
\textbf{Text-based (Logi. Reg.)} & 0.5224 (0.01) & 0.5275 (0.01) \\
\textbf{Text-based (SVM)} & 0.5510 (0.00) & 0.7673 (0.00) \\

\midrule
\textbf{Count-based LocalHealth} & & \\
MH only & 0.5052 (0.04) & 0.6195 (0.08) \\
FI only & 0.4465 (0.01) & 0.6788 (0.06) \\
MH and FI & 0.5133 (0.03) & 0.6384 (0.06) \\
General only & -- & -- \\

\midrule
\textbf{Text-based LocalHealth} & & & & \\
MH only & 0.5668 (0.02) & 0.6005 (0.02) \\
FI only & 0.5602 (0.01) & 0.6443 (0.02) \\
MH and FI & 0.5853 (0.02) & 0.6416 (0.03) \\
General only & 0.5984 (0.01) & 0.6676 (0.01) \\

\midrule
\textbf{Count-based LocalHealth with ADI} & & & & \\
MH-only & 0.5647 (0.12) & 0.6936 (0.04) \\
FI only & 0.5545 (0.13) & 0.7157 (0.04) \\
MH and FI & 0.6138 (0.10) & 0.6931 (0.03) \\
General only & -- & -- \\

\midrule
\textbf{Text-based LocalHealth with ADI} & & & & \\
MH only & 0.7089 (0.04) & 0.7452 (0.05) \\
FI only & 0.7117 (0.03) & 0.7536 (0.04) \\
MH and FI & 0.7085 (0.03) & 0.7433 (0.04) \\
General only & 0.7236 (0.02) & 0.7648 (0.03) \\

\midrule
\textbf{Text-based LocalHealth with ADI and Sentiment} & & & & \\
MH only & 0.7013 (0.03) & 0.7358 (0.04) \\
FI only & 0.7133 (0.02) & 0.7529 (0.03) \\
MH and FI & 0.6895 (0.03) & 0.7205 (0.04) \\
General only & 0.7254 (0.02) & 0.7639 (0.03) \\

\bottomrule
\end{tabularx}
\end{table}


==> tables/table_result_3_extended.tex <==
% table_result_3.tex

\begin{table}
\caption{\textbf{Effect of Text Encoder.} }
\centering
\begin{tabularx}{\linewidth}{cccccc}
\toprule
\textbf{Language Model} & \textbf{Trainable Par.} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Accuracy}  \\
\midrule

Majority baseline & -- & 0.2471 & 1.0000 & 0.3962 & 0.2471 \\
ADI only & -- & 0.6421 (0.14) & 0.7194 (0.12) & 0.6406 (0.11) & 0.7281 (0.05) \\
RoBERTa-base [33] & 120 & 0.7189 (0.01) & 0.7735 (0.01) & 0.7236 (0.02) & 0.7648 (0.03) \\
RoBERTa-large [33] & 330 & 0.7192 (0.01) & 0.7801 (0.01) & 0.7228 (0.02) & 0.7604 (0.03) \\
Twitter-RoBERTa-base [12] & 120 & 0.7210 (0.01) & 0.7771 (0.01) & 0.7245 (0.02) & 0.7644 (0.04) \\
Twitter-RoBERTa-Sentiment-base [12] & 120 & 0.7182 (0.01) & 0.7696 (0.03) & 0.7185 (0.02) & 0.7620 (0.03) \\
PHS-BERT [6] & 330 & 0.7242 (0.01) & 0.7823 (0.01) & 0.7301 (0.02) & 0.7697 (0.03) \\


\bottomrule
\end{tabularx}
\end{table}
